On the Hardness of Dominant Strategy Mechanism Design

We study the communication complexity of dominant strategy implementations of combinatorial auctions. We start with two domains that are generally considered "easy": multi-unit auctions with decreasing marginal values and combinatorial auctions with gross substitutes valuations. For both domains we have fast algorithms that find the welfare-maximizing allocation with communication complexity that is poly-logarithmic in the input size. This immediately implies that welfare maximization can be achieved in ex-post equilibrium with no significant communication cost, by using VCG payments. In contrast, we show that in both domains the communication complexity of any dominant strategy implementation that achieves the optimal welfare is polynomial in the input size. We then move on to studying the approximation ratios achievable by dominant strategy mechanisms. For multi-unit auctions with decreasing marginal values, we provide a dominant-strategy communication FPTAS. For combinatorial auctions with general valuations, we show that there is no dominant strategy mechanism that achieves an approximation ratio better than $m^{1-\epsilon}$ that uses $poly(m,n)$ bits of communication, where $m$ is the number of items and $n$ is the number of bidders. In contrast, a \emph{randomized} dominant strategy mechanism that achieves an $O(\sqrt m)$ approximation with $poly(m,n)$ communication is known. This proves the first gap between computationally efficient deterministic dominant strategy mechanisms and randomized ones. En route, we answer an open question on the communication cost of implementing dominant strategy mechanisms for more than two players, and also solve some open problems in the area of simultaneous combinatorial auctions.

==> general.tex <==
\section{A Hardness Result for Semi-Simultaneous Mechanisms}
\label{sec-general}

In this section we prove that semi-simultaneous mechanisms for combinatorial auctions with general valuations cannot provide a good approximation ratio, thus concluding the proof of Theorem \ref{theorem-general-impossibility}. 



\begin{theorem}
	\label{theorem-semi-simultaneous-impossibility}
Fix some $\eps>0$.
Let $\mathcal M$ be a deterministic normalized semi-simultaneous mechanism for combinatorial auctions with \magenta{$n=\Omega(m^{2-\epsilon})$} bidders with general valuations. 
Assume that
the approximation ratio of $\mathcal M$ is better than $m^{1-3\eps}$. Then, \sout{the number of bits that each player sends in $\mathcal M$} \magenta{there exists a set of valuations in which all values are polynomially related, such that the communication complexity of $\mathcal M$ when the input is from this set} is least $poly(\frac {2^{m^{\frac {\eps^2} 2}}} n)$. 
\end{theorem} 

Fix a mechanism $\mathcal{M}$ together with the dominant strategies $\mathcal{S}_1,\ldots,\mathcal{S}_n$ \sout{and set of general valuations}. 
By Lemma \ref{minimal-lemma}, we assume that $\mathcal{M}$ is minimal \magenta{with respect to a set of valuations which we will shortly define}. Our goal is to show that \magenta{there exists a set of polynomially related valuations such that} if $\mathcal M$ provides an approximation ratio of $c$ \magenta{with $x$ bits}, then there is a simultaneous algorithm (not necessarily incentive compatible) that provides an approximation ratio close to $c$ on the hard distribution of Section \ref{sec:simul} \magenta{with $poly(x,m)$ bits}. \shirinote{TODO - handle the fact the we need two levels of restriction, as in the email I sent to Shahar (if I understood things correctly)}
%\shirinote{It sounds here also like the proof of Theorem \ref{theorem-semi-simultaneous-impossibility} depends on the proof in Section \ref{sec:simul}}
 Note, however, that we heavily use the fact that $\mathcal M$ is deterministic, that is, provides an approximation ratio of $c$ in every instance. In particular, we will use the fact that $\mathcal M$ provides an approximation ratio of $c$ also in instances that are not in the support of the hard distribution.
 \magenta{Given an instance from the hard distribution $(u_1,\ldots,u_n)$, we construct an instance and use it to find an allocation
 	which is an (almost) $c$-approximation for the optimal welfare in $(u_1,\ldots,u_n)$.}
% 	 analyze the approximation ratio of $\mathcal M$ on it.} 
\sout{In the proof we construct various instances and analyze the approximation ratio of $\mathcal M$ on them.}
	 
	 \magenta{We assume that the mechanism $\mathcal{M}$ is minimal with respect to the following set of valuations:}
	 The domain of possible valuations of player $i$ is the domain of valuations of player $i$ in the hard distribution of Section \ref{sec:simul}, except that each valuation will have a weight  \magenta{$\alpha$ and noise $\epsilon$, that is negligible compared to $\alpha$}. That is, if \sout{$v$} \magenta{$u$} is a possible valuation of player $i$ in the hard distribution then we consider valuations \sout{$v'=\alpha \cdot v$} \magenta{$v=(\alpha+\epsilon) \cdot u$} for any weight $\alpha \cancel{\geq 0}$ \magenta{that is a power of $2$} and $\epsilon \in \{\magenta{0,}\frac \alpha {4^m}, \frac {2\cdot \alpha} {4^m}, \frac {3\cdot \alpha} {4^m}, \ldots,  \frac {3^m\cdot \alpha} {4^m}\}$.
	 Note that this random noise does not significantly change the approximation ratio of any instance and that the number of bits needed to describe a valuation has increased by only $poly(m)$ bits. To simplify the presentation, we often omit this random noise from the description of the valuation.
	  However, we note that in the instances that we \sout{consider} \magenta{construct} the valuations are not necessarily correlated in the same way as in the hard distribution. 
%	 \magenta{Also, we assume that the domain of each player includes the all-zero valuation.}
	  \shirinote{TODO - make sure that there are no zero valuations in the proof!! }
%Our goal here is to prove hardness for deterministic mechanisms, and hence we can assume that the mechanism performs well on every possible instance.

%, the valuations of the players (``random valuations'') will be very similar to the valuations considered in the hard instance of Section \ref{sec-simultanous-general}. There will be two main changes. The first is that the valuations of the players will not be necessarily correlated. The other is that each valuation will have a weight. That is, if $v$ is a random valuation then the weight of a valuation $v'=\alpha\cdot v$ is $\alpha$.


Concretely, in the proof we construct \emph{random base valuations} for player $i$ with a base set $T_i$, $|T_i|=2\cdot m^\eps$.  
By this we mean that the valuation is sampled from the distribution that chooses $t=2^{\Theta(\epsilon^2\cdot m^\epsilon)}$ valuable sets, each of size $m^\eps$ independently and uniformly at random from $T_i$, \magenta{and gives a value of $1$ to all of them. We call these sets the \emph{minimal non-zero sets} of a valuation}.

 Recall that an instance the hard distribution of Section \ref{sec-simultanous-general} satisfies that the players are partitioned into groups, where half of the base set of the players each group $j$ is disjoint from all other base sets and half of it is a shared set $B$ which we call the ``center''. Given a player in group $j$,  the disjoint half of his base set is called \emph{the special set}. 
 
 Each group $j$ has a random family $\mathcal A_j$ of sets of size $m^\eps$, and each bidder $i$ in the group is interested in a set from  $\mathcal{A}_j$  (i.e., gives it a value of $1$) with probability $\frac 1 m$. See Section~\ref{sec:simul} for the formal construction. Note that every valuation in any instance of the support of the hard distribution can be thought as a random base valuation. 


%The base set $T_i$ is shared among players in the same ``group''. In addition, all the base sets for all groups contain . (See Section~\ref{sec:simul} for more details.)

\sout{
We add some small random noise to all valuations that are considered here. Specifically, for a valuation with weight $\alpha$ we set the value of every set with value $\alpha$ to $\alpha+\eps$, where for each valuation $\eps$ is chosen uniformly and independently from the set $\{\frac \alpha {4^m}, \frac {2\cdot \alpha} {4^m}, \frac {3\cdot \alpha} {4^m}, \ldots,  \frac {3^m\cdot \alpha} {4^m}\}$. Note that this random noise does not significantly change the approximation ratio of any instance and that the number of bits needed to describe a valuation has increased by only $poly(m)$ bits. To simplify the presentation, we often omit this random noise from the description of the valuation.
}


%Consider the first non-trivial round of the mechanism that is, the first round in which there is some player $i$ that his dominant strategy is to send one message when his valuation is $v$, and a different one when his valuation is $v'$. Without loss of generality, we assume that the first non-trivial round is the first round since the messages that the players send in the previous rounds are always the same and thus can be ignored. 

\begin{lemma}\label{lemma-first-round}
There exists a set $A$ of consecutive powers of $2$, $|A|=O(\log m)$, such that for every player $i$ and for every base set $T_i$,  the following holds with probability at least $1-\frac 1 {exp(\magenta{m^{\eps})}}$: let $u_i$ be a random base  valuation of player $i$ with base $T_i$. Then, there exist some consecutive powers of $2$, $\alpha,\alpha'\in A$, and two noises $\epsilon,\epsilon'$ (as defined above) 
%\magenta{and $\eps,\eps'$} 
such that the message that player $i$ sends in the first round of $\mathcal M$ when his valuation is $(\alpha+\epsilon)\cdot u_i$ is different from the message he sends in the first round  when his valuation is $(\alpha'+\epsilon')\cdot u_i$. 


%\shirinote{Not clear enough that the probability is over the random valuation.}



\end{lemma}

Before proving this lemma (Subsection \ref{subsec-first-round-proof}) we show that it implies Theorem \ref{theorem-semi-simultaneous-impossibility} by constructing  a simultaneous algorithm for the hard distribution. 
%\shirinote{Again, the use of Section \ref{sec-simultanous-general} does not seem conceptual at all.}
% Recall that here we are ruling out only deterministic mechanisms (unlike Section~\ref{sec:simul} which considers randomized algorithms as well). Hence we will make an extensive use of the fact that $\mathcal M$ must provide a good approximation on \emph{every} instance in the support of the hard distribution, as well as on instances that are not in the support.

Consider valuations $u_1,\ldots, u_n$ that are sampled from the hard distribution. 
The guarantee of Lemma \ref{lemma-first-round} holds with high probability for a random base valuation of a single player $u_i$,
so by the union bound with high probability  the lemma holds for all $n$ valuations. We condition our analysis on the following event: \shirinote{TODO - Make sure that the valuations notations $v$,$u$ are consistent throughout the proof.}\magenta{For every player $i$, $u_i$ satisfies that it has $\alpha' = 2\alpha$ as in Lemma \ref{lemma-first-round}. For such $u_i$, we say that $\alpha$ is the \emph{critical} value for $u_i$ (if there are several values of $\alpha$ for which the lemma holds, choose one arbitrarily).} 
%For each random base valuation \sout{$v_i$} \magenta{$u_i$} for which $\alpha' = 2\alpha$ as in Lemma \ref{lemma-first-round} exists, we say that $\alpha$ is the \emph{critical} value for \sout{$v_i$} \magenta{$u_i$} (if there are several values of $\alpha$ for which the lemma holds, choose one arbitrarily). 
Divide the valuations of each player $i$ to $|A|$ sets $\{Q^i_{\alpha}\}_{\alpha\in A}$, where we put the valuation \sout{$v_i$} \magenta{$u_i$} of player $i$ in $Q^i_{\alpha}$ if $\alpha$ is critical for \sout{$v_i$} \magenta{$u_i$}. The fraction of valuations which are not in any set $Q^i_\alpha$ is negligible, by Lemma~\ref{lemma-first-round}. For a valuation $u_i$ with critical value $\alpha$, we denote the weights and the noises of the valuations with the different messages guaranteed by Lemma \ref{lemma-first-round} with high probability with $\alpha,\alpha'$ and with $\epsilon,\epsilon'$, respectively. 
%$v_i=(\alpha+\epsilon)\cdot u_i$ and with $v_i'=(\alpha'+\epsilon')\cdot u_i$. 
 %\shirinote{Don't we say twice the same thing, regarding the usage of Lemma \ref{lemma-first-round}?}

Based on the assumed semi-simultaneous mechanism $\mathcal{M}$, we construct a simultaneous algorithm.
The message that player $i$ with valuation $\cancel{v_i} \magenta{u_i}\in Q^i_{\alpha}$ sends 
%\magenta{in the simultaneous approximation algorithm} 
consists of several blocks:
\begin{enumerate}
\item The message he sends in the first round of $\mathcal{M}$ when his valuation is $(\alpha+\epsilon)\cdot u_i$. \shirinote{What we mean by that is $\mathcal{M}$ when restricted to the weights of $A$ plus some noise, right?}
\item The message he sends in the first round of $\mathcal{M}$ when his valuation is $(\alpha'+\epsilon')\cdot u_i$.
\item His base set (with probability $1-\frac 1 {exp(m)}$ each player can identify his entire base set by taking the union of all the sets he is interested in, since an item appears in a set with probability $\frac 1 2$ and there are exponentially many sets).
\item The index of $\alpha$ in $A$ ($O(\log\log m)$ bits) 
as well as $poly(m)$ bits that specify the value of the random noises $\epsilon,\epsilon'$. 
%\shirinote{To ask Shahar - why is it necessary?}
\end{enumerate}


We will see that if each player sends this message then we can construct a good simultaneous algorithm for the hard distribution. Towards this end, consider a distribution of instances $\mathcal I_\alpha$, defined for every $\alpha\in A$ as follows:
\begin{enumerate}
\item Sample an instance $(u_1,\ldots, u_n)$ from the hard distribution.
\item For each player $i$, if $u_i\in Q^i_{\alpha}$ (in this case we say that player $i$ is a \emph{participant}), the valuation $v_i$ of player $i$ is either $(\alpha+\epsilon)\cdot u_i$ or $(\alpha'+\epsilon')\cdot u_i$, each independently with probability $\frac 1 2$.
\item The valuation $v_i$ of every non-participant player $i$ is \magenta{$\frac{\alpha}{m^{2}}\cdot u_i$ (if $m^2$ is not a power of $2$, take instead the minimal power of $2$ that is larger than $m^2$)}.  
\end{enumerate}
\magenta{Our algorithm will sample uniformly at random $\alpha\in A$,}
\sout{For each $\alpha\in A$} and then will simulate the first round of $\mathcal{M}$ on an instance (very close to) $I_\alpha$ in the support of $\mathcal I_\alpha$. 
\magenta{We stress that $I_\alpha$ is constructed according to the messages sent by the players in the simultaneous algorithm, it is not sampled at random from $\mathcal{I}_\alpha$.} 


If participant $i$ does not send his special message in the first round for an instance \magenta{$I_\alpha$} \sout{in the support of $\mathcal I_\alpha$} we say that it is \emph{active} in that instance. Note that for every $\alpha\in A$, the messages that the players send in the simultaneous algorithm suffice to determine the participants in every instance in the support of $\mathcal I_\alpha$ as well as the messages that they send in the first round of the mechanism $\mathcal{M}$. 
%\sout{For each $\alpha\in A$, our simultaneous algorithm will simulate the first round of $\mathcal{M}$ on an instance $I_\alpha$ in the support of $\mathcal I_\alpha$.} 

We will use Claim \ref{claim-candidate} to identify many of the players that have significant contribution to the welfare in each such instance $I_\alpha$. We will then use this knowledge to produce an allocation with an approximation ratio comparable to that of $\mathcal{M}$, but with only one simultaneous round. We start with the following claim:
\shirinote{What's the goal of this paragraph? What is the goal of the distribution $\mathcal I_{\alpha}?$ I think we should write that its goal is to construct an algorithm for the hard distribution}
\begin{claim}\label{claim-positive-profit}
For every $\alpha\in A$ and instance $I_\alpha$ in the support of $\mathcal I_\alpha$, the probability that there is a player that is allocated a set with non-zero value and the profit of this player is $0$ is at most $\frac {n} {3^n}$.
\end{claim} \shirinote{Same noisy issue as the issue in Lemma \ref{lemma-first-round}}
\begin{proof}
Consider some player $i$ with valuation $v_i$ in the instance $I_\alpha$. By the taxation principle, for every bundle $S$ there exists a price $p_S$ (that does not depend on $v_i$) such that if all players play their dominant strategies, player $i$ is assigned a bundle $T$ in $\arg\max_S v_i(S)-p_S$. Recall that all bundles with non-zero value of player $i$ have the same value (denoted $y_i$). Let $p_i$ denote the minimal price of a bundle that player $i$ has a non-zero value for (so  by the taxation principle, $p_i$ is the price that player $i$ pays if he wins a bundle with non-zero value). Since $p_i$ does not depend on $v_i$ and since, fixing the value of $\alpha$, $y$ has $3^n$ possible values, the probability that $y_i=p_i$ is at most $\frac 1 {3^n}$. By the union bound, the probability that there is some player $i'$ with $y_i=p_i$ is at most $\frac n {3^n}$, and the claim follows.
\end{proof}
%The next claim shows that in every instance $\mathcal I_{\alpha}$ we can  almost all of the active participants that get a bundle that they are interested in.

\begin{claim}\label{claim-candidate}\shirinote{TODO - change statement to include $1-\frac{1}{\exp(m^\epsilon)}$}
For every $\alpha\in A$ and instance $I_\alpha$ in the support of $\mathcal I_\alpha$, with probability at least $1-\frac n {3^n}$ the following holds: consider the set $G$ of active participants in $I_\alpha$. Let $t$ be the number of players in $G$ that $\mathcal{M}$ allocates a \magenta{non-zero} set \sout{that they are interested in} to. Then, the special sets and the messages that the players send in the first round of $\mathcal M$ suffice to find a set $H$ of players that includes at least $t-1$ of these players. Moreover, $H$ includes at most one player from each group.
\end{claim}

\begin{proof}
Recall that the mechanism ``commits'' on the profit of an active player in $\mathcal{M}$ right after the first round (Corollary \ref{cor-commit-profit}). With probability $1-\frac n {3^n}$ all players who are assigned non-zero value sets have positive profit (Claim \ref{claim-positive-profit}), and we condition our analysis on that event happening.



%Since we add random noise to the valuations, if the maximum profit of a set with a non-zero value is non-negative, then it is strictly positive with high probability. Thus, every player that is allocated a set that he is interested in will have a positive profit with high probability. Recall that the valuable sets for players from the same group are intersecting, hence at most one player in a group can have a positive profit and get allocated a set that he is interested in. 
%\shirinote{I think that we need to explain why the fact that a player wins a bundle with the message of his non-noisy valuation implies that he wins also with his noisy valuation. If I understand correctly, I think that a possible explanation can use Corollary \ref{cor-commit-profit}}

%We begin by explaining why we can assume that the profit of an active player that wins a set that he is interested in is positive. 
%Let $v$ be the valuation of the active player. 
%Recall that the mechanism is normalized, so if the valuation $v$ has a zero profit, it means that the price of the set he is interested in is equal to his value. Since we add random noise to valuations, 
%If the profit of player $i$ with valuation $v$ is 
% 
%Recall that the mechanism ``commits'' on the profit of an active player in $\mathcal{M}$ right after the first round (Corollary \ref{cor-commit-profit}). Let $v_i$ be a valuation such that player $i$ is active and wins  and let $v_i'$ be a noisy version of it.  
%Let $v,v'$ with the same weight and with the same $u_i$ that differ on 


We now prove that almost all of those players can be identified after the first simultaneous round. We say that player $i$ that sends a message $X$ in the first round is a \emph{candidate} if there is a \emph{candidate valuation} $u_i\in Q^i_{\alpha}$ under which player $i$ sends the same message $X$ and has a positive profit for the special set (this implies that $u_i$ gives a non-zero value for the special set). 


We claim that there can be at most one candidate player in each group: suppose that there are two candidate players from the same group, $i$ and $i'$, and  denote their candidate valuations with $v_i$ and $v'_i$. Consider the instance $I''_\alpha$ that is obtained from $I_\alpha$ by replacing the valuation of player $i$ to $v_i$ and the valuation of player $i'$ to $v'_i$. Note that since the messages of the players are the same, the set of active players has not changed, and in particular $i$ and $i'$ are still active. Thus, both players have to be allocated a set with non-zero value. However, this is impossible because in the hard distribution all non-zero value sets of the players from the same group intersect \magenta{with probability at least $1-\frac{1}{\exp(m^\epsilon)}$}.

Note that a candidate player can be identified with no additional communication by checking whether there is a valuation for which player $i$ sends the message $X$ and is interested in his special set.

The only players that might get a set with non zero value but are not candidates are those who get a set with non-zero value that intersects with the center. However, in instances in the support of the hard distribution there can be at most one such player. Let the set of candidates be the set of players $H$ from the statement. The claim follows.
\end{proof}


We now describe the allocation of the simultaneous algorithm. Recall that the players send their base sets in the first round, thus we can identify  the center and  the special set of each player after the first round. 

The allocation of the simultaneous algorithm is as follows: we choose uniformly at random 
\shirinote{Not uniformly at random, we say that there exists an $\alpha$ with good enough probability}
 $\alpha\in A$ and apply Claim  \ref{claim-candidate} on $I_\alpha$ to obtain a set $H_\alpha$ of players  with at most one player from each group. $H_\alpha$ includes all but one of the active participants that are allocated a set with non-zero value. The simultaneous algorithm allocates each player that is included in $H_{\alpha}$ his special set. All other players are allocated no items at all.

%Recall that the optimal welfare of an instance in the hard distribution is $m^{1-\eps}$. 
We now express the approximation ratio of the simultaneous algorithm as a function of the approximation guarantee $c$ of $\mathcal{M}$.

\begin{claim}\label{claim-expected-special-message}
In a random instance sampled from $\mathcal I_\alpha$, let $S$ be the set of players who are interested in their special sets. Then, in expectation, at least half of the players $i\in S$ do not send their special messages (that is, are active).
\end{claim}
\begin{proof}
Fix some player $i\in S$ and the strategies of the other players. By Lemma \ref{lemma-first-round} and since $\alpha$ is critical for $v_i$, player $i$ sends a different message when his valuation is $\alpha\cdot v_i$ and when it is $\alpha'\cdot v_i$ (in both valuations the player is interested in his special set). Since we fix the messages of the other players, only one of the messages can be special (since the mechanism is semi-simultaneous). Thus player $i$ sends his special message with probability at most $\frac 1 2$. By linearity of expectation, we expect that at most half of the players in $S$ send their special messages, as needed.
\end{proof}

We can identify many of active participants that are allocated sets that they are interested in. Our worry now is that much of the welfare is due to non-active participants (non-participants do not contribute to the welfare because they have a zero valuation). To avoid this, we replace every valuation of a non-active participant to guarantee that this participant is not interested in his special set.
%\shirinote{Does the algorithm use $I_\alpha$ or a diluted version of $I_\alpha$?}
\begin{definition}
Fix $\alpha\in A$ and let $I_\alpha$ be an instance in the support of $\mathcal I_\alpha$. An instance $I'_\alpha$ is a \emph{diluted} version of $I_\alpha$ if it can be obtained by replacing the valuation of each non-active participant $i$ in $I_\alpha$, such that his valuation $v_i$ contains his special set, by a valuation $v'_i$ that does not contain the special set but the message that player $i$ sends is identical for both $v_i$ and $v'_i$. The valuations of the rest of the players (non-active players that are not interested in their special set, active players, non participants) remain the same as in $I_\alpha$.
\end{definition}


\begin{claim}\label{claim-diluted}
Fix $\alpha\in A$ and sample an instance $I_\alpha$ from the distribution $\mathcal I_\alpha$. If $L<\frac {2^{\eps^2 m}} {m^2}$, the probability that a diluted version $I'_\alpha$ of $I_\alpha$ does not exist is at most $\frac 2 n$.
\end{claim}
\begin{proof}
	We want to prove an  upper bound on the probability that there exists a player who is a non-active participant and cannot be replaced. 
 By Claim \ref{claim-change-valuation} below, the probability that a specific valuation of a player $i$ who is interested in his special set cannot be replaced is at most $\frac 2 {n^4}$. However, we replace only valuations of participants so it could be that such valuations are harder to replace.
 
	Recall that player $i$ is a participant only if $u_i\in Q^i_\alpha$. We say that $Q^i_\alpha$ is \emph{significant} if the probability that a random base valuation of player $i$ belongs to $Q^i_\alpha$ is at least $\frac 1 {n^2}$.
	If player $i$'s $Q^i_\alpha$ is significant, then the probability that he has a valuation that cannot be replaced given that he is a \emph{participant} is at most (by Bayes theorem)  $n^2\cdot \frac 2 {n^4}=\frac 2 {n^2}$. If player $i$'s $Q^i_\alpha$ is not significant, then the probability that he is a participant is below $\frac 1 {n^2}$, so clearly the probability that he is a participant and cannot be replaced is smaller or equal to $\frac 1 {n^2}$.

Thus, the probability that a single player needs to be replaced but cannot be is at most $\frac 2 {n^2}$. By the union bound over all the players, we get that the probability that a diluted version of $I_\alpha$ does not exist is at most $\frac{2}{n}$.
\end{proof}

%\begin{proof}
%	Note that for random valuations, the probability that a specific valuation of a player $i$ who is interested in his special set cannot be replaced is at most $\frac 2 {n^4}$. However, we replace only the valuations of active players and it could be that the valuations of active players are harder to replace. Recall that active players are by definition also participants. 
%	
%	In order to take this into account, we divide the players to two sets: a player is \emph{significant} if the probability that a random valuation of player $i$ belongs to $Q^i_\alpha$ is at least $\frac 1 {n^2}$, and otherwise it is \emph{negligible}. We want to upper bound for each player the probability that he is a non-active participant that cannot be replaced. 
%	
%	Assume that $i$ be a significant player. Then, we have that the probability that he cannot be replaced given that he is a participant is at most $n^2\cdot \frac 2 {n^4}=\frac 2 {n^2}$. 
%	 
%	By Claim \ref{claim-change-valuation} below, the probability that a valuation who wants its special set can be replaced is at most 
%	 $\frac 2 {n^4}$.  
%
%	
%	We say that $Q^i_\alpha$ is \emph{significant} if the probability that a random valuation of player $i$ belongs to $Q^i_\alpha$ is at least $\frac 1 {n^2}$. By Claim \ref{claim-change-valuation} below, the probability that a specific valuation of a player $i$ who is interested in his special set cannot be replaced is at most $\frac 2 {n^4}$. However, we replace only the valuations of participant players. If player $i$'s $Q^i_\alpha$ is significant, then the probability that a specific valuation of \emph{participant} $i$ that is interested in his special set cannot be replaced is at most (by Bayes theorem) $n^2\cdot \frac 2 {n^4}=\frac 4 {n^2}$. 
%	
%	
%	By the union bound, the probability that we can replace the valuations of all such players can be bounded by the sum of the probabilities that for each player $i$ we have that $Q^i_\alpha$ is significant plus the sum of probabilities that the valuation of each player $i$ can be replaced: $n\cdot \frac 1 {n^2} + n\cdot \frac 4 {n^2} = \frac 1 n + \frac 4 n = \frac 5 n$.
%\end{proof}
%


\begin{claim}\label{claim-change-valuation}
Let $T$ be some base set and let $\mathcal A_j$ be a family of $t = 2^{\Theta(\epsilon^2 m^\epsilon)}$ subsets of size $m^{\eps}$ of $T$ such that each subset is sampled uniformly at random. Let $v$ with a base set $T$ be the random base valuation in which player $i$ is interested in a subset from $\mathcal A_j$ with probability exactly $\frac 1 m$. Choose one of the $k$ sets independently at \shirinote{what is $k$?} random to be the special set. If $L<\frac {2^{\Theta(\eps^2 m^\epsilon)}} {n^4}$, with probability at least $1-\frac {2} {n^4}$, there is another valuation $v'$, with the same weight $\alpha$ of the valuation $v$, in which the player is not interested in this special set and the messages sent by $v$ and $v’$ in the first round of the mechanism $\mathcal M$ are the same.
\end{claim}
\begin{proof}
Fixing $T$ and the weight $\alpha$, we represent each valuation as in the statement by a $\{0,1\}^t$ vector that has $k=\frac t m$ coordinates that are equal $1$. The number of possible valuations is ${t \choose k}$.

Consider some $v$ that is interested in some set $S$. Suppose that for this specific $v$ there is no $v'$ as in the lemma. In other words, all vectors that send the same message as $v$ have a value of $1$ in the coordinate that corresponds to the set $S$. We say that this specific set $S$ is \emph{static} for the message.

A message is called \emph{dangerous} if there are at least $\frac k {n^4}$ static sets for it. Note that if a message is dangerous this implies that the location of $\frac k {n^4}$ coordinates with value $1$ is already determined. Therefore, the probability that a random base valuation makes the player send a specific dangerous message is at most $\frac 1 {m^{k/n^4}}$, since each of the static sets is chosen with probability $\frac{1}{m}$. Since the number of possible messages is at most $2^L$, the probability that we sample a random base valuation that sends some dangerous message is at most $2^L \cdot \frac 1 {m^k}$. Since $k=\frac t m$, for $L < \frac {k} {n^4} = \frac{2^{\Theta(\epsilon^2 m^\epsilon)}}{n^4}$, the probability that one player will send a dangerous message is exponentially small.

Conditioned on this event not happening (i.e., that the player does not send a dangerous message), the probability that the special set of a player is not static -- assuming that the player is interested in his special set -- is at least $1-\frac 1 {n^4}$, since each $1$ coordinate has the same probability of being a special set. The claim follows.
%
%
%
%
%
%
%
%
%
%
%
%A message is called \emph{dangerous} if it is static for at least $\frac {\frac k m} {n^4}$ sets. Note that if a message is dangerous this implies that the location of $\frac k {n^4}$ coordinates with value $1$ is already determined so the number of valuations that send a specific dangerous message is at most $r={t-\frac k {n^4} \choose k-\frac k {n^4}}$. If the length of the messages in the first round is $L$, then the number of valuations that send a dangerous message is at most $r\cdot 2^L$. The probability that a random valuation sends a dangerous message is therefore at most:
%\shirinote{Isn't it supposed to be $2^L \cdot \left (\frac {2k} t \right )^{\frac k {n^4}}$ instead of $2^L \cdot \left (\frac {2k} L \right )^{\frac k {n^4}}$ at the leftmost side of the inequality?}
%$$
%\frac {2^L \cdot {t-\frac k {n^4} \choose k - \frac k {n^4}}} {{t\choose k}} = \frac { \frac {2^L \cdot (t-\frac k {n^4})!} {(t-k)!(k-\frac k {n^4})!}} {\frac {t!} {k!(t-k)!}} = \frac {2^L (t-\frac k {n^4})! \, k!} {(k-\frac{k}{n^4})! \, t!} = \frac {2^L\cdot (k-\frac k {n^4}+1)\cdot (k-\frac k {n^4} +2) \cdot \ldots \cdot k} {(t-\frac k {n^4}+1)\cdot (t-\frac k {n^4} +2) \cdot \ldots \cdot t} < 2^L \cdot \left (\frac {2k} t \right )^{\frac k {n^4}}
%$$
%Recall that in the hard distribution we have $t=2^{\Theta(\eps^2 m^\epsilon)}$ and $k=\frac t m$, \shirinote{The probability that each set is chosen is $m$, so I guess the number of chosen sets is $\approx \frac{t}{m}$, but don't we need a concentration bound for that?} hence for $L < \frac {k} {n^4} = \frac{2^{\Theta(\epsilon^2 m^\epsilon)}}{n^4}$, the probability that one player will send a dangerous message is (doubly) exponentially small. Conditioned on this event not happening (i.e., that the player does not send a dangerous message), the probability that the special set of a player is not static -- assuming that the player is interested in his special set -- is at least $1-\frac 1 {n^4}$ \shirinote{why is it $1-\frac 1 {n^4}$, and not $1-\frac k {n^4}$?}, since each $1$ coordinate has the same probability of being a special set. The claim follows.
\end{proof}


The next two claims show that the optimal social welfare in diluted instances is linear in the number of participants that want their special sets that are satisfied. Thus, to provide a good approximation ratio the output allocation must satisfy many of these players.

\begin{claim}\label{claim-optimal-welfare}
Draw at random some instance $I_\alpha$ from $\mathcal I_\alpha$ and let $I'_\alpha$ be its diluted version, if it exists. The expected optimal welfare of $I'_\alpha$ is at least $\frac \alpha 2\cdot p_\alpha$, where $p_\alpha$ is the number of participants in $I_\alpha$ that want their special set.
\end{claim}
\begin{proof}
Consider all the participants in $I_\alpha$ that are interested in their special set. By Claim \ref{claim-expected-special-message} we expect half of them to be active. Note that the valuations of these players remain the same in $I_\alpha$ and $I'_\alpha$, since they are active in $I_\alpha$. The lemma follows since by construction their special sets are non-intersecting and each of them values his special set by at least $\alpha$.
\end{proof}

Recall that $c$ is the approximation ratio of $\mathcal M$. We now have that:
\begin{corollary}\label{cor-special-sets}
Draw at random some instance $I_\alpha$ from $\mathcal I_\alpha$ and let $I'_\alpha$ be its diluted version, if exists. In the instance $I'_\alpha$, the mechanism $\mathcal M$ must allocate at least $\frac {p_\alpha}{4c}-1$ of the players their special sets, where $p_\alpha$ is the number of participants in $I_\alpha$ that want their special set.
\end{corollary}
\begin{proof}
The approximation guarantee of the mechanism $\mathcal M$ is $c$, and the expected welfare is at least $\frac \alpha 2\cdot p_\alpha$, by Claim \ref{claim-optimal-welfare}. Thus the mechanism should output an allocation with welfare at least $\frac{\alpha}{2c} \cdot p_\alpha$.

Recall that all non-participants have valuations that are identically $0$ and that the weight of each participant player is either $\alpha$ or $\alpha'=2\alpha$. At most one participant can contribute a value of (at most) $\alpha'=2\alpha$ to the welfare without being allocated his special set.  Since each player who is assigned his special set can contribute at most $2\alpha$ to the welfare, and at most one player can be satisfied by a set that is not his special set, we have that the number of players that must be assigned their special set is at least:
$$
\frac {\frac \alpha {2c}\cdot p_\alpha  - 2\alpha} {2 \cdot \alpha} =  \frac { p_\alpha  } {4c} -1
$$ 
\end{proof}

All that is left now is to observe that since $|A|=O(\log m)$, there exists an $\alpha$ that contains a logarithmic fraction of the welfare. 


\begin{claim}
%Sample an instance from the hard distribution. The expected welfare of the allocation that the simultaneous algorithm outputs is at most $\frac {m^{1-2\eps}} {c}$.
With probability at least ... the expected welfare of the allocation that the simultaneous algorithm outputs for an instance sampled from the hard distribution is at \sout{most} \magenta{least} $\frac {m^{1-2\eps}} {|A| \cdot c}$. \shirinote{Something clearly needs to be fixed here}
\end{claim}

\begin{proof}
For a random instance sampled from the hard distribution, Lemma \ref{lemma-first-round} does not apply with probability at most $\frac 1 {exp(m^{\eps})}$ and Claim \ref{claim-positive-profit} with probability at most $\frac n {3^n}$. By Claim \ref{claim-diluted}, $I_\alpha$ does not have a diluted instance $I'_\alpha$ with probability at most $1-\frac 2 n$. Thus, with probability at least $\frac 1 2$ none of these bad events happen. 

Let $p_\alpha$ be the number of players $i$ with valuation $v_i\in Q^i_\alpha$ that want their special set. 
\shirinote{$p_\alpha$ was already defined differently}
In the hard distribution we have that $\sum_{\alpha} p_\alpha=m^{1-\eps}$\magenta{$-1$}.  Thus the expected value of $p_\alpha$ (when $\alpha$ is chosen uniformly at random), is $\frac {m^{1-\eps}} {|A|}\geq \frac {m^{1-\eps}} {10\log m}$.


Thus, since the simultaneous algorithm uses the allocation obtained by Claim \ref{claim-candidate} for a randomly chosen $I_\alpha$ we have that the expected number of players that get their special sets is, by Corollary \ref{cor-special-sets} at least:
$$
 \frac 1 2\cdot \left (\frac {\frac {m^{1-\eps}} {10\log m}} {4c} -1\right )\geq \frac {m^{1-2\eps}} {c}
$$
%$$
% \frac 1 2\cdot \sum_{\alpha\in A}\frac {p_\alpha-2} {4c}\geq  \frac 1 2\cdot \frac {m^{1-\eps} -2|A|} {4c} \geq \frac {m^{1-2\eps}} {c}
%$$
\end{proof}

Recall that in the hard distribution the expected welfare of any simultaneous algorithm with short enough message length is at most $m^{\eps}$. We therefore have that:
$$
\frac {m^{1-2\eps}} {c} \leq m^{\eps}
$$
and thus $c\geq m^{1-3\eps}$, as needed.

\subsection{Proof of Lemma \ref{lemma-first-round}}\label{subsec-first-round-proof}

\begin{definition}
\label{def-neighboring}
%We say that two different valuations $w,w'$ with weights $\alpha, \alpha'$, respectively, are \emph{neighboring} if the following two conditions holds:
%\begin{enumerate}
%\item $\frac \alpha {\alpha'}\in \{\frac 1 2, 1, 2\}$.
%\item There exist items $j,j'$ such that there exists a one-to-one and onto correspondence $f$ between all but at most one of the minimal non-zero sets $S$ of $w$ and all but at most one of the minimal non-zero sets \magenta{$S'$} of $w'$ such that $w(S)=w'(S')$ and $S'=f(S) \setminus \{j\}+\{j'\}$.
%\end{enumerate}
%\shirinote{Comment about erased definition - I think that we need to explain better what we mean by "minimal non-zero set"}
	We say that two different valuations $w,w'$ with weights $\alpha, \alpha'$  
	respectively, are \emph{neighboring} if $\frac \alpha {\alpha'}\in \{\frac 1 2,1, 2\}$ and \emph{at most one} of the following conditions holds:
	\begin{enumerate}
%		\item $\alpha\neq \alpha'$.
%		\item $\epsilon \neq  \epsilon'$.    
		\item There exist items $j,j'$ such that we switch between them, in the sense such that for every subset $S$, either $w(S)=w'(S)$ or $w(S)=w'(S')$ where $S'=S-\{j\}+\{j'\}$.
		\item $w,w'$ differ only on one coordinate, i.e. 
		there exist a subset of items $T$ such that for every subset $S$ other than $T$, $w(S)=w'(S)$. 
	\end{enumerate} 
where the equality is up to noise, i.e. if $w(S),w'(S)$ have different noises then they are considered to be equal. 
\end{definition}


\begin{claim}\label{claim-neighboring}\shirinote{I think that it makes sense to say what is the set of valuations that we discuss. We talk about "base sets" so we discuss the valuations of the hard distribution, so we should mention it somewhere}
Fix some player $i$ and let $v,v'$ of player $i$ be two valuations that send different messages in the first round of the mechanism $\mathcal M$. Then, there are two neighboring valuations $w,w'$ of player $i$ that send different messages in the first round.
\end{claim}
\begin{proof}
	Note that since $\mathcal{M}$ is dominant strategies and minimal for the set of weighted random base valuations, so we can safely assume that $v,v'$ are random base valuations multiplied by some weight and noise. 
%	Note that the mechanism $\mathcal{M}$ is minimal with respect to all random base valuations, 
Denote the weights of $v,v'$ with weights $\alpha,\alpha'$ 
%\magenta{and noise $\epsilon,\epsilon'$} 
respectively. Assume without loss of generality that $\alpha'\geq \alpha$. Define a sequence of valuations $v=w_0, w_1, \ldots, w_k=v'$ as follows. Each valuation $w_r$ is obtained from the valuation $w_{r-1}$ by one of the following operations: first, $w_r=2\cdot w_{r-1}$ until the weight of $w_{r}$ is $\alpha'$.
%\magenta{Afterwards, if the noise of $w_{r-1}$ and $v'$ are different, add $\epsilon'-\epsilon$ to the noise of $w_{r}$.}
 Then, suppose that the base sets of $w_{r-1}$ and $v'$ are different ($T$ is the base set of $w_{r-1}$, $T'$ is the base set of $v'$). Obtain $w_{r}$ from $w_{r-1}$ by renaming some item $j\in T \setminus T'$ to some item $j'\in T' \setminus T$. When the bases of the valuations are the same but the valuations are not identical, there is at least one set $S$ such that
$w_{r-1}(S)\neq v'(S)$. Take such a set $S$ and define $w_r$ to be identical to $w_{r-1}$, except that $w_r(S)=v'(S)$. Similarly to Definition \ref{def-neighboring}, we consider values to be equal if they are equal up to noise.  
%\sout{$w_{r-1}(S)=\alpha'$ and $v'(S)=0$ and another set $S'$ such that $v(S')=\alpha'$ and $w_{r-1}(S')=0$.
%\shirinote{Why is it true? The number of non-zero sets for a valuation is not fixed..} Define $w_r$ to be the valuation in which all minimal sets that the valuation $v$ gives non-zero value to are the same except that the set $S'$ replaces $S$.}

By construction, each pair of valuations $w_r,w_{r+1}$ consists of neighboring valuations. Since the messages that $w_0$ and $w_k$ send are not the same, there must be one pair $w_r,w_{r+1}$ in which each valuation sends a different message. The claim follows since $w_r,w_{r+1}$ are neighboring valuations.
%
%
%We first find some two valuations $u,u'$ of player $i$ that their weights are either the same or differ by a factor of $2$, that send different messages in the first round.
%
%
%Suppose that $\alpha> \alpha'$ (if they are equal there is nothing to prove). Obtain a valuation $v'_{\2\cdot \alpha'}$ by multiplying all values of $v'$ by $2$. If the message that $v$ sends is different than the message that $v'_{\2\cdot \alpha'}$ sends then we have found two valuations that send different messages that their weights differ by a factor of $2$. If the message remain the same we continue obtaining new valuations by multiplying the weight until we obtain the valuation $v'_{\alpha}$. If the message that one of the valuations that we obtained has changed then we are done as in the previous case. Else, the messages that $v$ and $v'_{\alpha}$ send in the first round are not the same and they have the same weight, as needed.
%
%Thus, from now on we may assume that $v$ and $v'$ share the same weight $\alpha$, up to a multiplicative factor of $2$. The first case is when both valuations belong to the support of the hard distribution on some set $T$. If differ by at most one minimal non-zero set then they are neighboring valuations (the correspondence $f$ is the identity function) and we are done. Otherwise, there is one set $S$ such that $v(S)=\alpha$ and $v(S)=0$ and another set $S'$ such that $v(S')=\alpha'$ and $v(S')=0$. We obtain a new valuation $v''$ in which all minimal sets that the valuation $v$ gives non-zero value to are the same except that the set $S'$ replaces $S$. If $v''$ and $v$ send different messages then we are done. Otherwise, we continue similarly gradually obtaining new valuations that are ``closer'' to $v'$ until a different message is sent or until the newly obtained valuations differs from $v'$ by only one minimal non-zero set.
%
%If the valuations belong to the support given different sets ($T$ for $v$, $T'$ for $v'$), we obtain new valuations by renaming some item $j\in T-T'$ to some item $j'\in T'-T$. If the message changes then we are done, otherwise we continue the process until $|T-T'|=|T'-T|=1$. We then change the non-zero minimal sets similarly to the previous case, until we obtain two neighboring valutions with different messages in the first round.
\end{proof}
\sout{Let $v,v'$ be two neighboring valuations of some player $i$ that send different messages in the first round, as guaranteed by Claim \ref{claim-neighboring}. Let $\alpha$ be the weight of $v$ and $\alpha'$ the weight of $v'$. }
	%Define $A=\{\frac \alpha {m^3}, \frac {2\alpha} {m^3}, \frac {4\alpha} {m^3}, \ldots, \alpha', \alpha,\ldots \frac {m^3\cdot \alpha} 2 ,m^3\cdot \alpha \}$. Observe that $A=O(\log m)$.

We say that a player is \emph{insensitive} with respect to some valuation $v$ and a set $A$ if for every $\alpha\in A$ a player with valuation $\alpha\cdot v$ sends the same message in the first round of the mechanism $\mathcal M$.

\begin{lemma}\label{lemma-random}
Let $v,v'$ be two neighboring valuations with weights $\alpha$ and $\alpha'$ of some player $i$ that send different messages in the first round of the mechanism $\mathcal M$. 
Let $T,T'$ be the base sets of $v,v'$ respectively. Let $W$ be some base set that is obtained by choosing \sout{at random} $\frac {|T|} 2$  items from $T\cap T'$ and $\frac {|T|} 2$ items arbitrarily.\footnote{$|T\cap T'|\ge |T|-1$ because $v,v'$ are neighboring.} Fix some player $i'\neq i$ and consider a random base valuation $w$ with a base set $W$. With probability at least $1-\frac 1 {exp(m^{\eps})}$ (
\sout{over the choice of half of the items in $W$ and} 
over the construction of the random base valuation given $W$), $w$ is sensitive in the set $A'=\{\frac \alpha {m^3}, \frac {2\alpha} {m^3}, \frac {4\alpha} {m^3}, \ldots, \alpha', \alpha,\ldots \frac {m^3\cdot \alpha} 2 ,m^3\cdot \alpha \}$.
\end{lemma}
\begin{proof}
	\sout{
Consider the random instance
 which is defined by player $i$ having valuation $v$ or $v'$ with probability $\frac 1 2$, player $i'$ has a random base valuation $w$ on the base set $W$ as in the statement of the lemma, and the rest of the players have valuations that are identically $0$.} 
% \shirinote{Why do we sample a random instance? Can't we just take a look directly at the instance of $v$. Also - don't we consider two instances, and show that the mechanism cannot give good approximation for both of them?}
We prove the lemma by describing two instances such that the mechanism $\mathcal M$ cannot give a good approximation for both of them it if $w$ is insensitive.
Fix the valuation of every player $i''\neq i,i'$ to be an arbitrary valuation with a very small weight of $\frac{\alpha}{2^m}$. 
If $w$ is sensitive in $A'$ we are done. Thus, assume that it is insensitive. 
%The instance is as follows: The valuation of player $i'$ is $w$, and the valuation of each player $i''\neq i,i'$ is an arbitrary random base valuation with a very small weight of $\frac{\alpha}{2^m}$.
%
%If $w$
%is sensitive in $A'$ we are done, thus  assume that it is insensitive.
Since the mechanism $\mathcal M$ is semi-simultaneous, given the message that player $i'$ sends for $w$ and the messages that the other players send for their valuations with small weight, player $i$ does not send his special message for either $v,v'$ because he sends different messages for them.  
%The valuation of player $i$ is either $v,v$
% The choice of the valuation of player $i$ is more involved.  
%Observe the the neighboring valuations $v,v'$ with weights $\alpha,\alpha'$ that player $i$ sends different messages for in the first round of the mechanism $\mathcal M$.  
%
%If $v$ has another valuation $v'$ that satisfies that 
 
%  and has weight $\alpha$ (but note that since $w$ is not sensitive in $A$ the message of player $i'$ is the same if as long as the weight belongs to the set $A'$). 
%  \shirinote{Is $\alpha$ a notation? Is it the $\alpha$ from the statement? If the latter one is correct, why can we assume it?}
%Since the mechanism $\mathcal M$ is semi-simultaneous, fixing $w$ (and the zero valuations of all other players except player $i$), player $i$ does not send his special message for at least one of $v$ or $v'$. 
Without loss of generality, suppose it is $v$. 
%\shirinote{It is not without loss of generality, because $w/v_{i'}$ is constructed according to he base set of $v$, not according to the base set of $v'$.}
Player $i$ does not send his special message, so by Corollary \ref{cor-commit-profit} his profit is determined after the first round. Because of the random noise we add to the valuations, with probability $1-\frac 1 {3^m}$ the profit of player $i$ is either strictly positive or all of his non-zero value sets have negative profit (the bad event is that the non-zero set with the maximal profit has zero profit, but this happens with small probability since the prices are only a function of the other players and do not depend on the random noise). \shirinote{I don't understand the point of the random noise. We fix a semi-simultaneous mechanism for valuations that are sampled from the hard distribution and have a weight $\alpha$ that is a power of $2$, and then we say that this mechanism also provides good approximation for the noisy valuations? Is this what we do?}

If player $i$'s profit is $0$, then the mechanism commits to allocating no items to him (the profit of all items that he is interested in is negative). Here we use the fact that the message that $i'$ sends remains the same when his weight is the lowest possible in $A'$. In this case the optimal welfare is at least $\alpha$ (by allocating player $i$ all items), but the mechanism outputs an allocation with welfare at most $\frac \alpha {m^3}$, which is the weight of player $i'$. The approximation ratio is only $m^3$.

The other case is when player $i$'s profit is positive and thus the mechanism commits on allocating player $i$ a set with value $\alpha$. Similarly to before, we observe that the message that $i'$ sends remains the same when his weight is the highest possible in $A'$. In this case the optimal welfare is at least $m^3\cdot \alpha$ (by allocating player $i'$ a set with non-zero value). However, note that with probability at least $1-\frac{1}{exp(m^\eps)}$ 
%\shirinote{Why $1-\frac 1 {n^\eps}$? TODO - figure out what bumber here makes sense }
 all non-zero value sets of player $i'$ intersect with all non-zero value sets of player $i'$ (since the base sets have large intersection), thus player $i'$ cannot be satisfied if player $i$ is satisfied. Therefore, the mechanism outputs an allocation with welfare at most $\alpha$, which is the weight of player $i$. The approximation ratio is only $m^3$.
\end{proof}

Lemma \ref{lemma-first-round} can now be deduced. 
$\mathcal{M}$ is minimal with respect to the random base valuations, so there exist two valuations $v_1,v_2$ with base sets $T_1,T_2$ that send different messages in the first round. By Claim \ref{claim-neighboring}, we can assume that $v_1,v_2$ are neighboring.  
%\shirinote{By Claim \ref{claim-neighboring}, neighboring valuations do not necessarily have the same base set.}
 We want to show that a  random base valuation $v'$ of player $i'$ with \sout{a randomly chosen} base set $T'$ is sensitive with high probability. Obtain a base set $T''$ by choosing at random half of the items of $T_1\cap T_2$ and half of the items of $T'$ (if $T_1\cap T_2\cap T'\neq \emptyset$ it might be need  to arbitrarily add more items to make sure that $|T''|=m^\eps$). Construct a random valuation $v''$ for player $i''\neq i,i'$ with base set  $T''$. By Lemma \ref{lemma-random}, with probability at least $1-\frac 1 { exp(m^{\eps})}$, $v''$ is sensitive for player $i''$ on $A'$. Let $\beta,\beta'$ be the two consecutive weights such that player  $i''$ sends a different messages when his valuation is $\beta\cdot v''$ and $\beta'\cdot v''$. Note that $\beta\cdot v''$ and $\beta' \cdot v''$ are neighboring, so by applying Lemma \ref{lemma-random} again we get that a random base valuation of player  $i'$  with a base set  $T'$ is sensitive on the set $A^{\beta}=\{\frac \beta {m^3}, \frac {2\beta} {m^3},  \ldots ,m^3\cdot \beta \}$  with 
 probability at least $1-\frac 1 {\exp(m^{\eps})}$. Since we have that $\frac \alpha {m^3}\geq \beta  \geq m^3\cdot \alpha $, we get Lemma \ref{lemma-first-round} for every player other than player $i$ with respect to the set $A=\{\frac \alpha {m^6}, \frac {2\alpha} {m^6}, \frac {4\alpha} {m^6}, \ldots, \alpha', \alpha,\ldots \frac {m^6\cdot \alpha} 2 ,m^6\cdot \alpha \}$.

Thus, we only need to prove that Lemma \ref{lemma-first-round} holds for player $i$. The proof for player $i$ is very similar to the above one. Fix a player $i$ with a random base valuation $v_i$ with base set $T_i$. 
Obtain a base set $T''$ by taking half of the items of $T_i$ and $\frac{|T_i|}{2}$ items arbitrarily. 
Let $v_{i''}$ be 
a random base valuation  for player $i''\neq i$ with base $T''$. Since we have proven Lemma \ref{lemma-first-round}
for all players except player $i$, we have that with probability $1-\frac 1 {\exp(m^{\eps})}$ $v_{i''}$ is sensitive with respect to the set  
$A''=\{\frac \alpha {m^6}, \frac {2\alpha} {m^6}, \frac {4\alpha} {m^6}, \ldots, \alpha', \alpha,\ldots \frac {m^6\cdot \alpha} 2 ,m^6\cdot \alpha \}$, so there exist two consecutive weights $\gamma,\gamma'\in A''$ such that player $i''$ sends different messages for in the first round of the mechanism $\mathcal{M}$ for $\gamma\cdot v_{i''}, \gamma'\cdot v_{i''}$. Observe that $\gamma\cdot v_{i''}, \gamma'\cdot v_{i''}$  are neighboring, so by  Lemma \ref{lemma-random} the  valuation $v_i$ is sensitive with respect to $\{\frac{\gamma}{m^3},\frac{2\gamma}{m^3},\ldots, m^{3}\cdot \gamma\}$ with probability $1-\frac 1 {\exp(m^{\eps})}$. Since $m^{6}\cdot \alpha \ge \gamma \ge \frac{\alpha}{m^6}$, we have that  Lemma \ref{lemma-first-round} holds for $\{\frac{\alpha}{m^9},\frac{2\alpha}{m^9},\ldots, m^{9}\cdot \alpha\}$.  


==> preliminaries-changed.tex <==
\section{Formalities and Basic Observations}\label{preliminaries}
%Throughout the paper, we handle mostly dominant strategy mechanisms that are not necessarily simultaneous. To prove lower bounds in this model, we need to get our hands dirty with the intricate details of the communication protocols that represent a mechanisms, i.e. what some player says at one vertex given one strategy or the other, what leaves can be reached from some vertex and so on. In this section, we specify some conventions and simple observations regarding dominant strategy mechanisms, that will come useful when analyzing them. 

In this section we discuss some basic properties of dominant-strategy mechanisms. For simplicity, when we talk about a fixed mechanism $\mathcal{M}$ together with its dominant strategies $S_1,\ldots,S_n$ we will slightly abuse notation: We say that player $i$ with valuation $v_i$ sends a message $z$ at vertex $r$ instead of saying that the dominant strategy of player $i$ with valuation $v_i$ is to send message $z$ in at vertex $r$. We also say that valuations $v_1\ldots,v_n$ reach a leaf of a protocol, instead of saying that the strategy profile $(S_1(v_1),\ldots,S_n(v_n))$ leads to it.   We postpone all proofs to the appendix (Section \ref{sec-basic-proof}).      

\subsection{Minimal Dominant Strategy Mechanisms}
Since our main interest in this paper is in impossibility results, in this section, we show that all dominant strategy mechanisms can be simplified without harming their dominant strategy equilibria for every set of valuations and without any communication burden. Thus, we can analyze the power of \textquote{minimal} dominant strategy mechanisms without loss of generality. Formally:
\begin{definition}
%	Let $\mathcal{M}$ be a mechanism and strategies $(S_1,\ldots,S_n)$ for a valuation set $V=V_1\times \cdots V_n$.
	We say that a mechanism $\mathcal{M}$ is \emph{minimal} with repsect to the strategies $(S_1,\ldots,S_n)$ and the valuations $V=V_1\times \cdots \times V_n$ if it satisfies the following properties:
	\begin{enumerate}
		\item There are no useless messages in the protocol, i.e. if some player $i$ can send some message in some particular vertex, we assume that it is a dominant strategy for some type $v_i$ to send this message. It immediately implies that every leaf in the protocol has valuations $(v_1,\ldots,v_n)$ such that the strategies $(S_1(v_1),\ldots,S_n(v_n)$ reach this leaf. \label{obs1}
	 \item 	 The root of the protocol tree, which we denote with $r$, has at least one player $i$ that has two valuations $v_i,v_i'\in V_i$  such that the strategies  $S_i(v_i)$ and $S_i(v_i')$ dictate different strategies at vertex $r$. \label{obs2}
	\end{enumerate} 
\end{definition}
\begin{lemma}\label{minimal-lemma}
	Let $\mathcal{M}$ be a dominant-strategy mechanism and strategies $(S_1,\ldots,S_n)$ that realize a  social choice function $f:V\to\mathcal{A}$ with communication complexity of $c$ bits.
	Then, there exists a \emph{minimal} mechanism $\mathcal{M}'$ and strategies $(S_1',\ldots,S_n')$ that realize $f$ in dominant strategies with at most $c$ bits. 
\end{lemma}

\subsection{Induced Trees of Mechanisms}
We now introduce the notion of induced trees and prove some simple properties of it. %This way of thinking about dominant strategies mechanisms will serve us later on. We analyze minimal dominant strategy mechanisms, and this is without loss of generality as we showed in Lemma \ref{minimal-lemma}. 
Consider some vertex $u$ in a minimal dominant strategy mechanism. Let $Z_{j,u}$ denote the set of possible messages that player $j$ can send at node $u$ (assume that $Z_{j,u}=\emptyset $ if player $i$ does not send any message at node $u$). Fix some player $i$ with $Z_{i,u}\neq \emptyset$ and some set of messages for the other players $z^u_{-i}=(z_1, \ldots,z_{i-1},z_{i+1},\ldots, z_{n})$ where each $z_j\in  Z_{j,u}$. The \emph{induced tree of $i$ at vertex $u$ given $z_{-i}^u$} is the tree that is rooted by $u$ and contains all subtrees that are connected to $u$ by an edge $(z_i,z^u_{-i})$ for every possible $z_i\in Z_{i,u}$. I.e., we fix the messages of all other players except player $i$ and think about each message $z_i$ as leading to the subtree that the set of messages $(z_i,z_{-i}^u)$ leads to. For an illustration,  see Figure \ref{my-third-tikz}.


\begin{figure}[H]
\centering 
\setlength{\belowcaptionskip}{-1pt}
\caption{Illustration of the subtree $u$ of a two-player protocol and one of its induced trees.
The vertex $u$ satisfies that $Z_1^u=\{z_1,z_1'\}$ and $Z_2^u=\{z_2,z_2'\}$,
i.e. each player has two possible messages.  The leaf $l$ that is labeled with $(A,p_1,p_2)$ satisfies that alternative $A$ is chosen, and that player $1$ pays $p_1$ and player $2$ pays $p_2$. The same holds for the leaf $l'$ with respect to its outcome $(A',p_1',p_2')$. The induced tree at \ref{subfig-induced} describes how the protocol looks like from the point of view of player $1$ when player $2$ sends the message $z_2$. 
}
\label{my-third-tikz}
\begin{subfigure}[b]{1.0 \linewidth}
	\centering
	\setlength{\belowcaptionskip}{-1pt}
	\caption{An illustration of the full tree protocol at vertex $u$.}
	\label{subfig-full-protocol}
	\begin{tikzpicture}
		\node[shape=circle,draw=black,minimum size=0.75cm] (r) at (1.5,1.5) {\small$u$};
\node[shape=circle,draw=black,minimum size=0.75cm] (v) at (-3,0) {\small$v$};
\node[shape=circle,fill=magenta!10,draw=black,minimum size=0.75cm,label=below:{\small $(A,p_1,p_2)$}] (l) at (-4,-1) {\small$l$};
%		\node[] (alloc) at (-1,-2.5) {$(m-s,v_a(m)-v_a(m-s))$};
\node[shape=circle,draw=black,minimum size=0.75cm] (v') at (6,0) {}; 
\node[shape=circle,draw=black,minimum size=0.75cm] (l') at (7,-1) {};
%		\node[] (bundle') at (3,-3) {$S_1',p_S'$}; 

\node[shape=circle,draw=black,minimum size=0.75cm] (n') at (5,-1) {}; 
\node[shape=circle,draw=black,minimum size=0.75cm] (n) at (-2,-1) {}; 

\node[shape=circle,draw=black,minimum size=0.75cm] (v-newl) at (0,0) {\small$v'$};
\node[shape=circle,draw=black,minimum size=0.75cm] (v-newl-kid-left) at (-1,-1) {};
\node[shape=circle,draw=black,,fill=magenta!50,minimum size=0.75cm,label=below:{\small $(A',p_1',p_2')$}] (v-newl-kid-right) at (1,-1) {\small$l'$};

\node[shape=circle,draw=black,minimum size=0.75cm] (v-newr) at (3,0) {};
\node[shape=circle,draw=black,minimum size=0.75cm] (v-newr-kid-left) at (4,-1) {};
\node[shape=circle,draw=black,minimum size=0.75cm] (v-newr-kid-right) at (2,-1) {};

%		\draw[thick,red!60] (-1.6,0.5) rectangle (1.45,-2) {};
%		\node[red!60] at (-0.9,0.7) {subtree $t$};
%		
%		\draw[thick,blue!60,anchor=mid west] (1.55,0.5) rectangle (4.7,-2) {};
%		\node[blue!60] at (4,0.7) {subtree $t'$};
%		


\draw [->] (r) edge  node[sloped, above] {\footnotesize $z_1,z_2$} (v);
\draw [->] (r) edge  node[sloped, above] {\footnotesize $z_1',z_2'$} (v');
\draw [->] (r) edge  node[sloped, below] {\footnotesize $z_1',z_2$} (v-newl);
\draw [->] (r) edge  node[sloped, below] {\footnotesize $z_1,z_2'$} (v-newr);
\draw [->] (v) edge[dotted]  node[sloped, above] {}  (l);
\draw [->] (v') edge[dotted]  node[sloped, above] {} (l');
\draw [->] (v) edge[dotted]  node[sloped, above] {} (n);
\draw [->] (v') edge[dotted]  node[sloped, above] {} (n');
\draw [->] (v-newl) edge[dotted] node[sloped,above] {} (v-newl-kid-left);
\draw [->] (v-newl) edge[dotted] node[sloped,above] {} (v-newl-kid-right);
\draw [->] (v-newr) edge[dotted] node[sloped,above] {} (v-newr-kid-left);
\draw [->] (v-newr) edge[dotted] node[sloped,above] {} (v-newr-kid-right);

%\draw (current bounding box.north east) rectangle (current bounding box.south west);

\end{tikzpicture}

\end{subfigure}
\vspace{2.0em}% Space between image A and B
\begin{subfigure}[b]{ 1.0 \linewidth}
	\centering
	\setlength{\belowcaptionskip}{3pt}
	\setlength{\abovecaptionskip}{3pt}
	\caption{The induced tree of player $1$ at vertex $u$ given the message $z_2$ of player $2$. 
%		An illustration of a protocol with two players, where a vertex $u$ satisfies that $Z_1^u=\{z_1,z_1'\}$ and $Z_2^u=\{z_2,z_2'\}$,
%		i.e. each player has two possible messages. The protocol tree at \ref{subfig-full-protocol} describes the subtree of the protocol whose root is vertex $u$. In particular, if the leaf $l$ is labeled with $(S_1,S_2,p_1,p_2)$ it means that the outcome is that player $1$ wins $S_1$ and pays $p_1$, whereas player $2$ wins $S_2$ and wins $p_2$. The same holds for the leaf $l'$ with respect to its outcome $(S_1',S_2',p_1',p_2')$.
	}	
	\label{subfig-induced}
\begin{tikzpicture}
	\node[shape=circle,draw=black,minimum size=0.8cm] (u) at (1.5,1.5) {$u$};
	\node[shape=circle,draw=black,minimum size=0.8cm] (v) at (0,0) {$v$};
%	\node[shape=circle,draw=black,minimum size=0.8cm] (l) at (-1,-1) {};
	\node[shape=circle,fill=magenta!10,draw=black,minimum size=0.8cm,label=below:{\small $(A,p_1)$}] (l) at (-1,-1) {\small$l$};
	\node[shape=circle,draw=black,minimum size=0.8cm] (v') at (3,0) {$v'$}; 
%	\node[shape=circle,draw=black,minimum size=0.8cm] (l') at (4,-1) {};
	\node[shape=circle,draw=black,,fill=magenta!50,minimum size=0.8cm,label=below:{\small $(A',p_1')$}] (l') at (4,-1) {\small$l'$};
	\node[shape=circle,draw=black,minimum size=0.8cm] (n') at (2,-1) {}; 
	\node[shape=circle,draw=black,minimum size=0.8cm] (n) at (1,-1) {}; 
	
	
	\draw [->] (u) edge  node[sloped, above] {\small$z_1$} (v);
	\draw [->] (u) edge  node[sloped, above] {\small $z_1'$} (v');
	\draw [->] (v) edge[dotted]  node[sloped, above] {}  (l);
	\draw [->] (v') edge[dotted]  node[sloped, above] {} (l');
	\draw [->] (v) edge[dotted]  node[sloped, above] {} (n);
	\draw [->] (v') edge[dotted]  node[sloped, above] {} (n');
\end{tikzpicture}

\end{subfigure}

\end{figure}

%We are now about to prove 
%We now explain and prove the property of \textquote{known prices}, which we will use repeatedly in our proofs. 
%Roughly speaking, it says that if at some vertex player $i$ has two messages that lead him to two different subtrees, and there exist leaves in each subtree that are labeled with the same allocation $S\subseteq M$ for him - those leaves are also labeled with the \emph{same price} for him. We now state and prove it formally. 
\begin{lemma}\label{containmentlemma}
	Fix some player $i$ \sout{with valuation $v$}, vertex $u$, and messages of the other players $z^u_{-i}$. Consider the induced subtree of player $i$ at vertex $u$ given $z^u_{-i}$. If the bundle $S$ appears in some subtree $t$ with price $p_S$ and a bundle $S'$ such that $S\subseteq S'$ appears in a different subtree $t'$ with price $p_{S'}$, then $p_{S'}\ge p_S$.
	%	\footnote{It could be that $S$ appears in the subtree $t$ with more than one price, and similarly $S'$ appear in the subtrees $t/t'$ with more than one price.} 
\end{lemma}
\begin{corollary}\label{knownpricescorollary}
Fix some player $i$ \sout{with valuation $v$}, vertex $u$, and messages of the other players $z^u_{-i}$. Consider the induced tree of player $i$ at vertex $u$ given $z^u_{-i}$. 
If the bundle $S$ appears in two different subtrees, then 
 all the leaves in this induced tree that are labeled with $S$ have the same payment for player $i$.\shirinote{I think that the valuation should not be in the statement of both the lemma and the corollary}
\end{corollary} 
For clarity, we state Lemma \ref{containmentlemma} and Corollary \ref{knownpricescorollary} for the setting of combinatorial auctions. However, both hold for any social choice function.

%\subsubsection{Properties of VCG Mechanisms} \label{vcg-subsec-prem}
%We now restrict ourselves to 2-player VCG mechanisms. Both our proofs of hardness for exact welfare rely heavily on this lemma, which is a direct application of Corollary \ref{knownpricescorollary} for VCG mechanisms. 
% 



%\begin{lemma}\label{knownpricelemma}
%	Fix a dominant strategies mechanism $\mathcal{M}$ together with its dominant strategies $(S_1,\ldots,S_n)$. 
%	Let player $i$ be a player such that $S_i(v_i)$ and $S_i(v_i')$ dictate at the root vertex $r$ different messages  $z_i,z_i'$. Fix the messages $z_{-i}=(m_1,\ldots,z_{i-1},z_{i+1},\ldots,z_{n})$ of the other players at vertex $r$. Denote the subtrees that $(z_i,z_{-i})$ and $(z_i',z_{-i})$ lead to with $t,t'$ respectively. 
%	Assume that there exist two leaves in the subtrees $t,t'$ which are labeled with the same allocation $T_i$ for player $i$. 
%	Then, all the leaves that belong to subtrees
%	that $z_{-i}$ lead to and are labeled with the allocation $T_i$ have the same payment for player $i$. 
%\end{lemma}
%\begin{proof}
%	Let $\ell,\ell'$ be two leaves in the subtrees $t,t'$ that are labeled with the same allocation $T_i$. 
%	Denote the prices of player $i$ at the leaves $\ell,\ell'$ with $p,p'$, respectively. 
%	By Lemma \ref{uselessrootlemma}, there are no useless messages, so there exist valuation profiles $(v_i,v_{-i}),(v_{-i}',v_{-i}')$ such that:
%	$$
%	(S_i(v_i),S_{-i}(v_{-i}))\to \ell,\quad
%	(S_i(v_i'),S_{-i}(v_{-i}'))\to \ell'
%	$$   
%	Observe the following strategy profile $s_{-i}$ of the players in $N/\{i\}$: at the root vertex $r$, send the messages $z_{-i}$.
%	At the subtree $t$, choose the actions specified by $S_{-i}(v_{-i})$, and at the subtree $t'$, choose the actions specified by $S_{-i}(v_{-i}')$.  Note that:
%	$$
%	(S_i(v_i),s_{-i})\to \ell,\quad
%	(S_i(v_i'),s_{-i})\to \ell'
%	$$
%$S_i(v_i)$ is dominant for the valuation $v_i$, so we have that $v_i(T_i)-p\ge v_i(T_i)-p'\implies p'\ge p$. Similarly, we have that $S_i(v_i')$ is dominant for the valuation $v_i'$, so $v_i'(T_i)-p'\ge v_i'(T_i)-p\implies p\ge p'$, so $p=p'$. Thus, all the leaves in $t$ and in $t'$ labeled with $T_i$ have the same price. By reusing the same argument, we get that every other leaf in a subtree that $z_{-i}$ leads to which is labeled with $T_i$ also has the same price.   
%\end{proof}
%Given a  mechanism coupled with dominant strategies $(G,S_1,S_3,\ldots,S_n)$, we define for each valuation $v_i\in \mathcal{V}_i$ a function $Profit_{v_i}:V_1\times\cdots V_n \to \mathbb{R}$ as the profit of a  player $i$ when her valuation is $v_i$ given the outcome of the mechanism $\mathcal{M}$ given the strategies $(S_i(v_i),S_{-i}(v_{-i}))$. 
%\begin{lemma}\label{unitedlemma}
%	Fix a  mechanism and strategies $(G,S_1,S_2)$
%	that realize it in dominant strategies. 
%	Let $r$ be the root of the protocol associated with the mechanism.  
%	Consider two sets of valuations $(v_1,\ldots,v_n)$ and $(v_1',\ldots,v_n')$ and a player $i$ such that:
%	\begin{enumerate}
%		\item The strategy $S_i$ dictates \emph{different} messages for $v_i,v_i'$ at the root vertex $r$.
%		\item The strategies $S_{-i}(v_{-i})$ dictate the \emph{same}  messages for $v_{-i},v_{-i}'$ at the root vertex $r$.
%	\end{enumerate}
%	Then,  $Profit_{v_i}(v_i,v_{-i})\ge Profit_{v_i}(v_i',v_{-i}')$.  
%\end{lemma}
%\begin{proof}
%	Denote the messages that  $S_i(v_i)$ and $S_i(v_i')$ dictate at vertex $r$   with $m_i$ and with $m_i'$ respectively. Denote the messages that $S_{-i}(v_{-i})$ and $S_{-i}(v_{-i}')$ dictate with $m_{-i}=(m_1,\ldots,m_{i-1},m_{i+1},\ldots,m_{i})$. 
%	
%	We denote with $t$ the subtree that $(m_i,m_{-i})$ reaches, and we denote with $v'$ the vertex  that $(m_i',m_{-i})$ reaches. 
%	We define a strategy $s_{-i}$ for the players in $N/\{i\}$ as follows: at vertex $r$, send the messages $m_{-i}$. At subtree $t$, choose the actions specified by $S_{-i}(v_{-i})$. For every other subtree, choose the actions specified by $S_{-i}(v_{-i}')$. 
%	
%	Let $\ell$ be the leaf that $(S_i(v_i),S_{-i}(v_{-i}))$ reaches, and let $\ell'$ be the leaf that $(S_i(v_i'),S_{-i}(v_{-i}'))$ reaches. 
%	Note that $(S_i(v_i),s_{-i})$ reaches the leaf $\ell$, and $(S_i(v_i'),s_{-i})$ reaches the leaf $\ell'$, so since $S_1(v_1)$ is a dominant strategy for player $i$ given the valuation $v_1$, we have $Profit_{v_i}(v_i,v_{-i})\ge Profit_{v_i}(v_i',v_{-i}')$.  
%\end{proof}
